On the tightness of the maximum of branching Brownian motion in random environment

We consider one-dimensional branching Brownian motion in spatially random branching environment (BBMRE) and show that for almost every realisation of the environment, the distributions of the maximal particle of the BBMRE re-centred around its median are tight as time evolves. This result is in stark contrast to the fact that the transition fronts in the solution to the randomised Fisher--Kolmogorov--Petrovskii--Piskunov (F-KPP) equation are, in general, not bounded uniformly in time. In particular, this highlights that -- when compared to the settings of homogeneous branching Brownian motion and the F-KPP equation in a homogeneous environment -- the introduction of a random environment leads to a much more intricate behaviour.

==> Makefile <==
#This is a empty makefile for TeX files
#Last Modified:		Tue 19 Nov 2013 19:30:38 CET
#By Jiri Cerny


#name of the main file without .tex
NAME = tightness

#files with pictures (not necessary to fill in)
PICFILES = 

#bibliography database
BIBFILES = $(HOME)/texty/Bibliografie/bib.bib

#additional texfiles, not $NAME.tex
OTHER_TEXFILES =

#index style file
MAKEINDEXSTYLE = 

#command flags
PDFLATEX = pdflatex
LATEXFLAGS = --synctex=1
DVIPSFLAGS =

#host modifications
HOSTNAME = $(shell uname)
include $(HOME)/texty/Tex_local.$(HOSTNAME).mk

######################################################
#you probably do not need to edit after this line

TEXFILES = $(NAME).tex $(OTHER_TEXFILES)


# Phony targets ########################################
.PHONY: archiv target dvi all ps pdf pspdf bib print clean mrproper scaled index

target: pdf

dvi: $(NAME).dvi

all: ps pdf 

ps: $(NAME).ps

pdf: $(NAME).pdf

pspdf: ps
	ps2pdf $(NAME).ps

scaled: scaled.$(NAME).pdf

bib: 
	touch $(BIBFILES)
	make pdf

index:  $(NAME).ind

print: ps
	lpr $(NAME).ps

archiv:
	mkdir -p archiv
	gzip -9 -c $(NAME).tex  >  archiv/$(NAME)$(shell date +"%y%m%d").tex.gz

clean:
	-rm -fv  *.aux *.bbl *.blg *.fls *.log *.nav *.out 
	-rm -fv  *.snm *.toc *.ilg *.idx *.ind *.fdb_latexmk
	-rm -fv  *.synctex.gz
	-rm -fv  *~ *.bak DEADJOE
	-rm -fv  .latexrun*

mrproper: clean
	-rm -iv *.dvi *.ps *.pdf

tags: $(NAME).aux $(BIBFILES) $(TEXFILES)
	ctags $(NAME).tex $(NAME).bbl

ps4pdf: pdf
	latex $(NAME).tex
	dvips -Ppdf -o $(NAME)-pics.ps $(NAME).dvi
	ps2pdf $(NAME)-pics.ps $(NAME)-pics.pdf
	$(PDFLATEX) $(NAME)


# Explicit rules ########################################
$(NAME).dvi: %.dvi:  %.tex %.bbl  $(PICFILES) $(OTHER_TEXFILES)
	-latex $(LATEXFLAGS) -interaction=scrollmode $(basename $@).tex
	@while grep 'cross-references' $*.log; \
		do latex $(LATEXFLAGS) -interaction=scrollmode $(basename $@).tex; \
	done

$(NAME).pdf: %.pdf: %.tex %.bbl $(PICFILES) $(OTHER_TEXFILES)
	$(PDFLATEX) $(LATEXFLAGS) -interaction=scrollmode $(basename $@).tex
	@while grep 'cross-references' $(basename $@).log; \
		do $(PDFLATEX) $(LATEXFLAGS) -interaction=scrollmode $(basename $@).tex; \
	done

#$(NAME).pdf: %.pdf: %.tex %.bbl $(PICFILES) $(OTHER_TEXFILES)
#	rubber -r $(HOME)/.config/rubber.conf -f --pdf -s $<
#	rubber-info -r $(HOME)/.config/rubber.conf --check $<

# Pattern rules ########################################
%.dvi:  %.tex 
	latex $(LATEXFLAGS) -interaction=scrollmode $(basename $@).tex
	@while grep 'cross-references' $*.log; \
		do latex $(LATEXFLAGS) -interaction=scrollmode $(basename $@).tex; \
	done

%.pdf: %.tex 
	$(PDFLATEX) $(LATEXFLAGS) -interaction=scrollmode $(basename $@).tex
	@while grep 'cross-references' $(basename $@).log; \
		do $(PDFLATEX) $(LATEXFLAGS) -interaction=scrollmode $(basename $@).tex; \
	done

#%.pdf: %.tex 
#	rubber -f --pdf -s $<
#	rubber-info --check $<

%.ind: %.idx
	makeindex -s $(MAKEINDEXSTYLE) $<

%.bbl: $(BIBFILES)
	-$(PDFLATEX) -draftmode $(LATEXFLAGS) -interaction=scrollmode $(basename $@).tex
	-bibtex $(basename $@)

%.ps: %.dvi
	dvips -t a4 $(DVIPSFLAGS) $<  -o $@

scaled.%.ps: %.ps
	pstops '1:0@1.25(-2.7cm,-5cm)' < $< > $@

scaled.%.pdf: %.pdf
	pdfjam --nup 2x1 --landscape --frame true --trim '1cm 2.0cm 1cm 1.0cm' --outfile $@ < $<


%.table: %.gnuplot
	gnuplot $<

